Ecosystem-level Analysis of Deployed Machine Learning Reveals Homogeneous Outcomes

Machine learning is traditionally studied at the model level: researchers measure and improve the accuracy, robustness, bias, efficiency, and other dimensions of specific models. In practice, the societal impact of machine learning is determined by the surrounding context of machine learning deployments. To capture this, we introduce ecosystem-level analysis: rather than analyzing a single model, we consider the collection of models that are deployed in a given context. For example, ecosystem-level analysis in hiring recognizes that a job candidate's outcomes are not only determined by a single hiring algorithm or firm but instead by the collective decisions of all the firms they applied to. Across three modalities (text, images, speech) and 11 datasets, we establish a clear trend: deployed machine learning is prone to systemic failure, meaning some users are exclusively misclassified by all models available. Even when individual models improve at the population level over time, we find these improvements rarely reduce the prevalence of systemic failure. Instead, the benefits of these improvements predominantly accrue to individuals who are already correctly classified by other models. In light of these trends, we consider medical imaging for dermatology where the costs of systemic failure are especially high. While traditional analyses reveal racial performance disparities for both models and humans, ecosystem-level analysis reveals new forms of racial disparity in model predictions that do not present in human predictions. These examples demonstrate ecosystem-level analysis has unique strengths for characterizing the societal impact of machine learning.

==> sections/03_hapi_polarization.tex <==
\section{Outcome Homogenization in Commercial ML APIs (HAPI)}
\label{sec:hapi-polarization}
To establish general trends in system-level behavior of deployed ML, we analyze a large-scale audit of commercial ML APIs \citep[\hapi;][]{chen2022hapi}.

\subsection{Data}
\label{sec:hapi-data}
\hapi releases the predictions of deployed ML models evaluated on standard AI benchmarks.
We work with a subset\footnote{For simplicity, we only work with datasets with a clear ground truth to remove ambiguity about what constitutes a failure -- a principle which we revisit in subsequent experiments on dermatology.} of these benchmarks: we consider eleven benchmarks that span three modalities (images, speech, text) and associated tasks (facial emotion recognition, spoken command recognition, sentiment analysis).
For each benchmark dataset and each instance (e.g. image, speech sample) $x_i$ therein, we consider the profile of outcomes $\textbf{y}_i$ to be the outcomes of three commercial ML APIs on the data point.
\kc{added 'instance' to address Percy's comment earlier.}
% Note for connor: lots of different conventions, but one is to use bold for vectors (since arrows look less pretty) and normal math mode for scalars. So the outcomes are normal and the profiles are mathbf. 
For example, on the \fluent dataset, the profile for data point $x_i$ is the outcomes from the three spoken command recognition models (Amazon, IBM, Google) $\textbf{y}_i = [{\hat{y}_i^{1}}, {\hat{y}_i^{2}}, {\hat{y}_i^{3}}]$, where ${\hat{y}_i^{1}}$ is the outcome from the most accurate model (Microsoft) and ${\hat{y}_i^{3}}$ is the outcome from the least accurate model (Google).
\hapi annually evaluated the same API endpoints to track how they change: we initially consider the 2020 results and later discuss trends over time (2020 -- 2022).

% \todo{Need to get response on issues with CMD dataset and Face++ 22 on AFNET}.

% Note for Connor - I reformatted the table and moved it to tables/basic_stats.table.tex. (feel free to ask me any questions!)
\input{tables/basic_stats_error.table}

% \subsection{ML APIs}
% \label{sec:apis}
% \todo{@Connor: Who uses APIs and for what? What APIs exist? How does usage diversify across different types of APIs? Which ones are the highest-stakes? The most frequently used? The most consequential (i.e. combining per-user stakes with frequency roughly)? What is the economic footprint? What is the business/pricing model? What are known strengths and weaknesses? How do these properties interplay with downstream outcomes? Do APIs pattern differently from public models (e.g. is there post-processing or other aspects of system/interface design you would not see in a normal research model)?
% Overall, we want a crisp and succinct characterization of APIs: a reader should be clear on why they should care.}

\subsection{System-level Behavior}
To ground the structure of the datasets and the performance of the models, we present basic statistics in \autoref{tab:basic-stats}.
Across most datasets, we observe that all three models achieve accuracies within 5--10\% of each other with some exceptions where the least accurate model $h^3$ is worse by a considerable margin (\digit, \yelp, \imdb). 
Interestingly, across almost all datasets, the systemic failure rate is roughly half the failure rate of the most accurate model $h^1$ (which is an upper-bound on the systemic failure rate: to be systemically failed, an individual must be failed by $h^1$). 

\paragraph{\PolarizedProfiles.}
To better understand systemic failures, we juxtapose the observed rates of systemic failures with a baseline of the rates we would observe if models made independent predictions at the instance level.
For example, the expected likelihood of systemic failure is simply the product of the models' failure rates.
More generally, under this assumption, the expected probability that a system-level profile exhibits exactly $t \in \{0, 1, \dots, k\}$ failures is given by the PMF of a Poisson-Binomial distribution parameterized by the $k$ model-specific failure rates. 
In \autoref{fig:digit_polarization}, we showcase the relationship between the observed and expected distributions for \digit as an exemplar.
We clearly observe that the observed distribution is more \textit{polarized} than expected: more instances are either exclusively failed or exclusively classified correctly than expected in \digit.
In fact, across all the datasets (\autoref{fig:polarization_all}), we see a very clear separation where the observed rate consistently exceeds the expected rate for either extreme, and the reverse holds for either intermediary profile (\ie 1 or 2 failures of the 3 possible). 

This suggests that model outcomes are not independent: a user is more likely to experience a \textit{universal success} or a \textit{systemic failure} than some intermediate outcome than the error rates of the models would suggest. 
% Rishi: We should weave in the point on monoculture at some point, but I don't think this is sufficient reason to posit concrete component-wise sharing (in fact, I am not sure I even think that is true here) or any direct form of monoculture. 
% We hypothesize that the disproportionate concentration of outcomes at the extremes is due to \textit{component sharing} \citep{bommasani2022picking}: most models tend to be similar in architecture and data and, therefore, likely struggle for the same types of inputs. 
This \polarization raises concerns that model systems are prone to succeed for the same type of user while simultaneously systemically failing for another type.

% \paragraph{Representing system outcomes.} A system level outcome for a single input $x^i$ represents the set of model outcomes on that input. Because we are dealing with classification tasks here, each outcome is either a correct prediction, henceforth 'success' and denoted as a 0, or an incorrect prediction, henceforth 'failure' and denoted as a 1. We represent a system outcome as a k-length list of model outcomes where k is the number of models. The $j_{th}$ element of the list represents the success or failure of model $m_j$ on that input. We order the models by their relative curacies such that $m_{j-1}$ is more accurate than $m_j$. 
% %%We need to say there is some x_i that we query all the models on. It would be good, at least for some things, to use macros. We order models such that m_1, m_k, s.t. i<j -. acc (m_i) < acc(m_j)
% We represent the entire system as a failure matrix: A failure matrix F is defined as an $N \times k$ matrix, where N represents the number of individuals and k represents the number of queried models. Each element of the matrix, $F[i,j]$, is a binary value that indicates if the $j_{th}$ model failed (1) or did not fail (0) for individual $i$. In other words, $F[i, :]$ is a k-length vector that represents the set of model outcomes on individual $i$.
%% Define a nxk matrix of failures. F \in {0,1},
% where f[i, :] is the vector of outcomes for a individual i
% 
% For example, consider an instance where $m_0$, the most accurate model, succeeds for the given input, but $m_1$ and $m_2$ -- the second to least and least accurate models -- fail for that input: we represent this as [0, 1, 1]. 
% At times, for simplicity, we may represent a system level outcome simply as the number of model that are correct for a given instance.
% In order to get a high level understanding of how model outcomes relate to each other, we first examine the observed distribution of system level outcomes compared to the distribution of system level outcomes we would expect if model outcomes were independent of each other. 

% Here, we represent system level outcomes simply as the number of models $[0, k]$ that correctly predict the label for that \instance. We count how many instances belong to each system level outcome and normalize by the total number of instances we observe. 

% We compare our observed distribution against the distribution we would expect if model outcomes were independent on each other: this distribution is represented by the Poisson binomial distribution parameterized by the error rates of the models: $[e_1, ..., e_k]$ where $k$ is the number of models queried.

% First, we build intuition on a single dataset, the DIGIT dataset, which contains spoken digit utterances: in \autoref{fig:digit_polarization}, we juxtapose the observed rates against the expected rates (assuming behavioral independence) for each possible system-level outcome. We find a clear distinction: the observed outcomes are more \textit{polarized} than we would expect under the assumption of independence. The observed rates, represented in dark, exceed the expected rates on the most extreme outcome profiles -- when 0 models or 3 models are correct -- while the opposite is true of the intermediate outcomes. 

% In \autoref{fig:polarization_all}, we find that this phenomonen holds across all the datasets that we examine: points above the line represent outcome profiles that occur more than expected while points below the line occur less than expected. We see that, across all datasets, extreme outcomes are above the line and therefore occur more often than expected while intermediate outcomes occur less often than expected -- mirroring the results from the DIGIT dataset. 

% This suggests that model outcomes are not independent, and a user is more likely to experience a \textit{universal success} or a \textit{systemic failure} rather than some intermediate outcome than the error rates of the models would suggest. We hypothesize that the disproportionate concentration of outcomes at the extremes is due to \textit{component sharing} \citep{bommasani2022picking}: most models tend to be similar in architecture and data and, therefore, likely struggle for the same types of inputs. This polarization raises concerns that model systems are prone to succeed for the same type of user while simultaneously systemically failing for another type.

% do a left figure with a single dataset to build intuition.
\begin{figure}
    \centering
    \begin{subfigure}[H]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/hapi/polarization_digit_22.png}
        \caption{Polarization for \digit dataset in 2022}
        \label{fig:digit_polarization}
    \end{subfigure}%
    \begin{subfigure}[H]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/hapi/polarization_all_datasets_22.png}
        \caption{Polarization for all considered datasets in 2022.}
        \label{fig:polarization_all}
    \end{subfigure}%
    \caption{Observed vs expected rate of system level outcomes for one dataset (a) and all datasets (b) in 2022. The expected rate is calculated under the assumption that model outcomes are independent of each other.}
\end{figure}





\subsection{Qualitative Findings}





\subsection{Takeaways}

==> sections/05_related_work.tex <==
\section{Related Work}
\label{sec:related-work}

==> sections/07_social_concerns.tex <==
\section{Social Concerns}
\label{sec:social-concerns}



==> sections/07_social_concerns_alternate.tex <==
\section{Social Concerns}
\label{sec:social-concerns}

\subsection{Users have fewer options in a homogeneous setting}

\begin{figure} 
    \centering
    \includegraphics[width=\columnwidth]{figures/hapi/polarization_change_in_proportion.png}
    \caption{\ct{I think we should move this figure and accompanying section (\autoref{sec:social-concerns} to appendix}The change in the probability of observing each other-model outcome with and without conditioning on $h_i$ failing. Conditioning on a single model failure significantly increases the probability of a user experiencing a systemic failure; this increase is greatest when the most accurate model in the system fails.}
    \label{fig:polarization_failures}
\end{figure}

Users have a reasonable expectation of choice when interacting with multiple models in a system: if one model fails for them, they should ideally have another option that could work for them. For example, if a consumer goes out and purchases an Amazon Echo but finds that Alexa, the speech system that underlies it, consistently makes mistakes for them, they could hope to go out and purchase a Google Nest or Apple HomePod. 

However, outcome homogenization, by concentrating failures on the same users, could reduce the probability that the Nest or the HomePod could work for them -- effectively shutting them out of the market. 

\paragraph{Experiment setup.} To test this hypothesis, we setup the following experiment. As before, let $F$ be the $N \times k$ failure matrix for a single dataset.
Define the submatrices $F_{-i} \in \{0,1\}^{N \times (k-1)}$ and $F_{-i}* \in \{0,1\}^{N_i \times (k-1)}$: $F_{-i}$ removes column $i$ from $F$ and $F_{-i}*$ further only includes the $N_i \leq N$ rows that $h^i$ failed on.
We juxtapose the profiles over $k-1$ outcomes in $F_{-i}$ with $F_{-i}*$ to demonstrate how system-level profiles change by conditioning on a data point being failed by $h_i$. Note here that the baseline case here, the profiles in $F_{-i}$, is a more stringent baseline than the one we used in \autoref{sec:hapi-polarization}: there, we used the expected outcome rates under the assumption of outcome independence; here, we use the true, observed outcome rates for the $k-1$ other models as the baseline.

\pl{did not expect experiment in this section, move to appendix?}

\paragraph{Impact of a single failure on the rate of systemic failure.} In \autoref{fig:polarization_failures}On average, when a single model fails for a user, that user is far more likely to experience a systemic failure compared to baseline probability that the user would have expected a systemic failure from the two other models. This effect is strongest when the most accurate model fails for the user, and weakest, though still statistically significant, when the least accurate model fails. This effect restricts the ability of failed users to seek alternative models when they confront a model failure and raises concerns that users can be functionally shut out of model-led systems. 

\rb{Write something about recourse/redress, Hima's work}

%  We calculate the observed distribution over the $2^{(k-1)}$ other-model outcomes in $F_i$. Our reference is the distribution of outcomes over the $2^{(k-1)}$ other-model outcomes \textit{without conditioning} on model $m_j$ failing. We then average these distributions across all (dataset, year, model) combinations to generate the average proportions across all the systems we observe.
% This exercise is motivated by how users might interact with deployed ML models in the real world: in the multi-interaction model, a user who is failed by a single model -- a hiring model, for example -- might interact with other hiring models by applying to additional jobs; in the single-interaction model, if a user is failed, we might ask the counterfactual of what would have happened had they chosen another model. In both of these cases, we want to understand how the other models in the system will perform on that user once we observe that the user has experienced that initial failure.


==> sections/08_predictors.tex <==
\section{Data-Centric Predictors of Homogenous Outcomes}
\label{sec:predictors}
Prior work has found that algorithmic monoculture and, more specifically, component sharing increases outcome homogenization in systems \citep{bommasani2022picking}. However, one might also posit that data-centric explanations account for homogenous outcomes: models could be expected to all fail for \textit{hard} examples and all succeed for \textit{easy} examples, or ambiguity in the instance label might lead models to collectively 'fail' for that instance. To examine this, we conduct two experiments: first, we examine how the 'ambiguity' of the label in \ferplus impacts the polarization effect; second, we examine how the performance of human dermatologists on an instance impacts the polarization of model-outcomes on those instances. 

\subsection{Ambiguous examples}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/hapi/polarization_by_ambiguity.png}
    % \caption{Observed vs. expected proportion of models correct for instances, grouped by the crowdsourcer disagreement percentage.}
    \caption{Utilizing the fact that labels for the \ferplus dataset are generated from the majority label of 10 crowdsourcer votes, we calculate the percentage of crowdsourcers that disagree with the majority label for each instance. We calculate observed vs \baseline distributions for instances, grouped by their disagreement percentage. The systemic failure rate is correlated with the disagreement percentage of the instance; however, outcome polarization exists across all groups. Instances with less disagreement (less ambiguity) have a lower difference between observed and \baseline rates but a higher ratio between the observed and \baseline rates.}
    \label{fig:polarization by ambiguity}
\end{figure}
    
One potential cause of homogenization might be the inherent ambiguity of the example: in the setting of facial emotion recognition, for example, humans might struggle to agree on the emotion since facial emotion recognition is inherently subjective. It could be possible that systemic failures occur more often than the \baseline because models all disagree with the ground-truth label on ambiguous examples. To examine the impact of ambiguous examples on outcome polarization, we use the \ferplus dataset which contains votes on the emotion label from 10 crowd-sourced taggers. We calculate the percentage of crowdsourcers who do not vote for the majority label for each \ferplus instance and examine the distribution of outcome profiles varies with the disagreement percentage of the instances.

\paragraph{Systemic failures are correlated with ambiguity, but polarization exists for all instance sets.} In \autoref{fig:polarization by ambiguity}, we find that, while the rate of systemic failure strictly monotonically increases as the level of crowdsourcer disagreement increases, the polarization effect exists regardless of the degree of disagreement. The strength of the polariztion effect varies with the degree of disagreement; however, whether it increases or decreases depends on how we measure the 'strength'. When interpreting the strength as the difference between the observed and \baseline rate, the strength of the effect increases as the rate of disagreement increases. However, when interpreting the strength as the ratio between the observed and \baseline rates, as in \citet{bommasani2022picking}, the strength is highest when the rate of disagreement is lowest. 

\subsection{Relationship between human accuracy and outcome homogenization in models}
\begin{figure}
  \centering
  \begin{subfigure}[b]{0.30\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/dermatology/rows=all,by=by_human_accuracy, cols=models, group=Humans both right.png}
    \caption{Subset of instances that both humans correctly predicted}
    \label{fig:both_humans_right}
  \end{subfigure}
  \hspace{3pt}%
  \begin{subfigure}[b]{0.3\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/dermatology/rows=all,by=by_human_accuracy, cols=models, group=1 human right, 1 human wrong.png}
    \caption{Subset of instances that one human incorrectly predicted}
    \label{fig:subfig2}
  \end{subfigure}
  \hspace{3pt}%
  \begin{subfigure}[b]{0.3\linewidth}
    \centering
    \includegraphics[width=\textwidth]{figures/dermatology/rows=all,by=by_human_accuracy, cols=models, group=Humans both wrong.png}
    \caption{Subset of instances that both humans incorrectly predicted}
    \label{fig:both_humans_wrong}
  \end{subfigure}
  \caption{We plot the observed distribution (darker color) of system-level outcomes from model predictions against what we would expect under the assumption that model outcomes are independent (lighter color). The left-most plot contains model predictions on the subset of instances where both human dermatologists correctly predicted the instance's label and the right-most plot contains model predictions on the subset of instances where both human dermatologists incorrectly predicted the label. We find that polarization correlates with human accuracy: we see very little polarization in \autoref{fig:both_humans_right}, but a fair deal of polarization in \autoref{fig:both_humans_wrong}.}
  \label{fig:by_human_accuracy}
\end{figure}

As a follow up to our work on \hapi, we examine the relationship in \ddi between human accuracy and model homogenization. We might hypothesize that homgenous outcomes result from the inherent 'difficulty' of an input. In \hapi, we didn't have a human-level assessment of the 'difficulty' of the inputs, so conducting this analysis was infeasible; in \ddi, however, we can take the collective accuracy of the two human dermatologists as a proxy for human-level difficulty. 

If human error and model homogenization were correlated, we could expect the following pattern: when both humans fail, we could expect models to systemically fail more than the baseline; when humans diverge in error (e.g. one correct and one incorrect), we could expect models to diverge more than expected; when humans are both correct, we could expect models to universally succeed more than expected. 

In \autoref{fig:by_human_accuracy}, we observe is more nuanced than this: we indeed find that when both humans fail, then models are more likely than expected to both fail. However, we also find that, when both humans fail, models are also more likely to universally succeed than expected. This is counter-intuitive; we would expect both models to fail more than expected, but it's unclear why they should succeed more than expected. 

When humans diverge in accuracy, we don't see that models are more likely to diverge than expected; instead, models are more likely to either both succeed or both fail than expected -- though the effect is weak.

Perhaps most surprisingly: when we condition on both humans being correct, instead of seeing both models also succeed at higher than expected rates, we essentially see no difference in observed vs expected rates for any system-level outcome -- suggesting that model outcomes behave as if they were independent of each other, a pattern we have never seen in any other model-system.





==> tables/basic_stats.table.tex <==
\begin{table*}[htp]
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cccc|ccc|cccc}
\toprule
 & \multicolumn{4}{c}{\textbf{Facial emotion recognition}} & \multicolumn{3}{c}{\textbf{Spoken command recognition}} & \multicolumn{4}{c}{\textbf{Sentiment analysis}} \\
 &   rafdb &    afnet &    expw & ferplus &  fluent &  digit &  amnist &    shop &    yelp &    imdb &  waimai \\
\midrule
\textbf{$h^1$ accuracy } &    0.72 &     0.72 &    0.73 &    0.84 &    0.98 &   0.78 &    0.99 &    0.92 &    0.96 &    0.86 &    0.89 \\
\textbf{$h^2$ accuracy } &    0.66 &     0.68 &    0.65 &    0.68 &    0.97 &   0.74 &    0.98 &    0.91 &    0.89 &    0.78 &    0.85 \\
\textbf{$h^3$ accuracy } &    0.61 &      NaN &    0.62 &    0.68 &    0.92 &   0.53 &    0.96 &    0.88 &    0.51 &    0.52 &    0.82 \\
\textbf{Systemic failure rate} &   0.152 &    0.211 &   0.181 &   0.066 &    0.01 &  0.129 &   0.002 &   0.039 &   0.021 &   0.043 &   0.065 \\
\textbf{Number of examples} &  15.3k &  287.4k &  31.5k &    6.4k &  30.0k &   2.0k &  30.0k &  62.8k &  20.0k &  25.0k &  12.0k \\
\textbf{Number of classes} &       7 &        7 &       7 &       7 &      31 &     10 &      10 &       2 &       2 &       2 &       2 \\
\bottomrule
\end{tabular}}
\caption{\textbf{Basic statistics on \hapi datasets.} 
To ground our understanding of \hapi, we provide basic information on the dataset structure, the accuracies of all models evaluated on the dataset, and the observed systemic failure rate (\ie fraction of instances misclassified by all models) in 2022, the most recent year for which we have data.
\rb{@Connor: Make the accuracies 3 decimal places to match sys fail rate. Probably can make the number of examples 2 digits (e.g. 15k, 290k, 6.5k but this is fine. Also should typeset the dataset names and use macros for each so we can use consistently throughout the paper}
\rb{Maybe switch the accuracies to errors?}
}
\label{tab:basic-stats}
\end{table*}
